Deep TEN: Texture Encoding Network

We propose a Deep Texture Encoding Network (Deep-TEN) with a novel Encoding Layer integrated on top of convolutional layers, which ports the entire dictionary learning and encoding pipeline into a single model. Current methods build from distinct components, using standard encoders with separate off-the-shelf features such as SIFT descriptors or pre-trained CNN features for material recognition. Our new approach provides an end-to-end learning framework, where the inherent visual vocabularies are learned directly from the loss function. The features, dictionaries and the encoding representation for the classifier are all learned simultaneously. The representation is orderless and therefore is particularly useful for material and texture recognition. The Encoding Layer generalizes robust residual encoders such as VLAD and Fisher Vectors, and has the property of discarding domain specific information which makes the learned convolutional features easier to transfer. Additionally, joint training using multiple datasets of varied sizes and class labels is supported resulting in increased recognition performance. The experimental results show superior performance as compared to state-of-the-art methods using gold-standard databases such as MINC-2500, Flickr Material Database, KTH-TIPS-2b, and two recent databases 4D-Light-Field-Material and GTOS. The source code for the complete system are publicly available.

==> related.tex <==
%-------------------------------------------------------------------------
\section{Related Work}

\begin{comment}

\begin{figure}[t]
\begin{center}
\includegraphics[height=1.0\linewidth]{figure/pipeline.eps}
\end{center}
\caption{ 
Pipeline of traditional dictionary learning and encoding includes multiple steps:
feature extraction, dictionary learning, feature encoding (pooling) and
classification.
}
\label{fig:pipeline}
\end{figure}
\end{comment}

% the material and texture work
Numerous methods have been developed for  texture and material modeling recognition,
including material recognition 
in-the-wild \cite{bell13, bell15, cimpoi15,li2012recognizing}, 
in-lab or controlled conditions
\cite{dana99,leung2001representing,zhang15,zhang16,DeGol16},  
descriptions \& attributes\cite{schwartz2013visual,cimpoi14,schwartz2015automatically}, 
and texture synthesis\cite{
efros1999texture,wei2000fast,lin2015visualizing,li2016precomputed}.
In early material recognition work, 
texture is represented by modeling the distribution of
local appearance. 
Local visual appearance are usually captured by the 
filter banks responses~\cite{dana97,leung2001representing,Cula01b, varma2003texture,geusebroek2003fast}.
%Those hand-engineered filters are designed to capture some low-level features such as edges, borders and corners~\cite{geusebroek2003fast}. 
The filter bank responses are then clustered into visual 
centroids (codewords), and texton distribution framework 
aggregates the hard-assignment weights 
as one variation of
Bag-of-Words (BoWs) representation~\cite{csurka2004visual}.
Recently deep learning features (pre-trained CNNs)
have outperformed the hand-engineered features
 and encoding residuals 
has been shown more effective than encoding assigning weights~\cite{jegou2011product}.
VLAD-CNN~\cite{gong2014multi} and FV-CNN~\cite{cimpoi15} encode pre-trained
CNN into an off-the-shelf representation
have shown the robustness as feature representation.


\begin{comment}
Dictionary learning is usually achieved by modeling the feature distributions, 
such as hard-assignment grouping of K-means~\cite{lloyd1982least} 
and a probabilistic version of Gaussian Mixture Model 
(GMM)~\cite{perronnin2007fisher},
or minimizing the reconstruction error
such as K-SVD~\cite{aharon2006img} and the other sparse coding algorithms.

learning general CNN features? reuse or share convolutional layer


\end{comment}


\begin{comment}
%Per-pixel, texton boost (extremely slow)
Previous work (Cimpoi 14, 15) solve this problem in two separate
steps: generating region proposals and classify the materials.
The accuracy is limited by the region proposal algorithms and 
the features are not helping generating proposals.

Region proposal

RGB-M camera.
\end{comment}
